Tempered, Anti-trunctated, Multiple Importance Sampling

Importance sampling is a Monte Carlo method that introduces a proposal distribution to sample the space according to the target distribution. Yet calibration of the proposal distribution is essential to achieving efficiency, thus the resort to adaptive algorithms to tune this distribution. In the paper, we propose a new adpative importance sampling scheme, named Tempered Anti-truncated Adaptive Multiple Importance Sampling (TAMIS) algorithm. We combine a tempering scheme and a new nonlinear transformation of the weights we named anti-truncation. For efficiency, we were also concerned not to increase the number of evaluations of the target density. As a result, our proposal is an automatically tuned sequential algorithm that is robust to poor initial proposals, does not require gradient computations and scales well with the dimension.

==> algo_graphs.tex <==
 \begin{tikzpicture}[auto,
  decision/.style = { diamond, aspect=2, draw=blue, thick, fill=blue!10,
    text width=5em, text badly centered,
    inner sep=1pt, rounded corners },
  block/.style    = { rectangle, draw=blue, thick, 
    fill=blue!10, text width=11.5cm, text centered,
    rounded corners, minimum height=2em },
  line/.style     = { draw, thick, ->, shorten >=2pt },
  ]
  \matrix [column sep = 5mm, row sep = 10mm] { %
    & \node [block] (start) {Start with a proposal distribution $q_1(\cdot)$ as a mixture
      parametrized with $\theta_1$ and set $t=1$}; &
    \\
    & \node (debutboucle) {}; &
    \\
    & \node [block] (draw) {\textbf{Draw} a sample of size $N_t$, $x_{t, 1}$, \ldots,
      $x_{t,N_t}$, from $q_t(x)$\\}; &
    \\
    & \node [block] (weight) {Compute the un-normalized \textbf{weights}
      $w_{t,1},\ldots, w_{t,N_t}$ as in \eqref{eq:weights} and
      $\ESS_t = (\sum_i w_{t,i})^2/\sum_iw_{t,i}^2$}; &
    \\
    \node(null3){}; & \node [decision] (ESS) {Is $\text{ESS}_t>\text{ESS}_\text{targeted}$?}; &
    \node [text width=5em] (stop) {\textbf{Stop}, recycle and return the results};
    \\
    & \node [block] (calibrate) {\textbf{Calibrate} $\beta_t$ with \eqref{eq:calibrate_beta}
      and $s_t$ with \eqref{eq:s}}; &
    \\
    % & \node [block] (Target) {Set new \textbf{target} by computing with transformed weights $\tilde{\omega}_{t,i}(\beta_t)=\widetilde{\omega_{t,i}^{\beta_t}}$  with \eqref{eq:calibrate_beta}}; &
    % \\
    & \node [block] (EM) {\textbf{Update} $\theta_{t}$ to set
      $\theta_{t+1}$ and the new proposal by
      performing a few steps of the
      \textbf{EM algorithm} on data $x_{t,1}$, \ldots,
      $x_{t,N_t}$ resampled with weights $\widehat w_{t,i}^{\beta_t}$ as in
      \eqref{eq:hat_w} 
    }; &
    \\
  };

  \begin{scope} [every path/.style=line]
    \path (start)        --    (draw);
    \path (draw)      --    (weight);
    \path (weight)   --   (ESS);
    \path (ESS) -- node [near start] {yes} (stop);
    \path (ESS) -- node [near start] {no} (calibrate);
    %\path (calibrate)   --   (Target);
    %\path (Target)   --   (EM);
    \path (calibrate) -- (EM);
    \path (EM)   --++  (-8,0)  |- (debutboucle) node [near end] {$t\to t+1$};
    \path (ESS)   --    node [near start] {yes} (stop);
  \end{scope}
  %
  % % legend for subprocedures
  % \node (leyend) at (7.5, 5){
  %   \begin{tabular}{>{\sffamily}l@{: }l}
  %     \multicolumn{2}{c}{\textbf{subprocedures}} \\
  %     DoAE & direction of arrival estimation     \\
  %     UID  & user identification                 \\
  %     DoAT & DoA tracking                        \\
  %     BF   & beam forming                        \\
  %     SF   & spatial filtering
  %   \end{tabular}
  % };
  % %
  % % legend for input and output variables
  % \node (leyend) at (7, 0){
  %   \begin{tabular}{l@{: }l}
  %     \multicolumn{2}{c}{\textbf{variables}}              \\
  %     DoA                       & direction of arrival    \\
  %     $\mathbf{i}$              & identification sequence \\
  %     $\mathbf{X},\,\mathbf{x}$ & signal model            \\
  %     DoA$_{\mathrm{T}}$        & DoAs up to date         \\
  %     $\hat{x}(t)$              & fitered signal
  %     \end{tabular}
  % };
\end{tikzpicture}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
